InjecGuard: Benchmarking and Mitigating Over-defense in Prompt Injection Guardrail Models

Prompt injection attacks pose a critical threat to large language models (LLMs), enabling goal hijacking and data leakage. Prompt guard models, though effective in defense, suffer from over-defense -- falsely flagging benign inputs as malicious due to trigger word bias. To address this issue, we introduce NotInject, an evaluation dataset that systematically measures over-defense across various prompt guard models. NotInject contains 339 benign samples enriched with trigger words common in prompt injection attacks, enabling fine-grained evaluation. Our results show that state-of-the-art models suffer from over-defense issues, with accuracy dropping close to random guessing levels (60%). To mitigate this, we propose InjecGuard, a novel prompt guard model that incorporates a new training strategy, Mitigating Over-defense for Free (MOF), which significantly reduces the bias on trigger words. InjecGuard demonstrates state-of-the-art performance on diverse benchmarks including NotInject, surpassing the existing best model by 30.8%, offering a robust and open-source solution for detecting prompt injection attacks. The code and datasets are released at https://github.com/leolee99/InjecGuard.

==> sections_ARR_submission/1-introduction.tex <==
\section{Introduction}\label{sec_intro}
Prompt injection attacks~\cite{perez_ignore_2022,greshake_not_2023,liu2024automatic} represent a serious and emerging threat to the security and integrity of \textit{large language models} (LLMs)~\cite{brown_language_2020}. These attacks exploit the models’ reliance on natural language inputs by inserting malicious or manipulative prompts, leading to undesirable behaviors such as goal hijacking or sensitive data leakage. For instance, a well-known prompt injection technique involves instructing the LLM to "ignore previous instructions,"~\cite{branch2022evaluatingsusceptibilitypretrainedlanguage,harang2023securing,perez_ignore_2022,pi_against_gpt3} which can override built-in safeguards and enable the execution of unauthorized actions. As the deployment of LLMs continues to expand across industries, the risk posed by prompt injection attacks becomes more pronounced, demanding effective and efficient defense mechanisms.

To address it, prompt guard models~\cite{promptguard,protectai,deepset,fmops} have recently been proposed as a promising solution.  These models work by analyzing the semantic meaning of the input data to detect malicious intent before it reaches the LLM. Unlike LLM models, prompt guard models are lightweight and computationally efficient, as they do not require the high inference cost associated with LLMs. Additionally, these models operate independently, without the need for victim LLM’s responses, further reducing computation costs compared to approaches like LLM guardrails~\cite{inan2023llamaguardllmbasedinputoutput}. These attributes make prompt guard models adaptable to various environments, and an attractive solution in scenarios where speed and resource optimization are critical.

\begin{figure*}[t!]
\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering    
    \includegraphics[width=0.95\textwidth,trim=0 0 0 0,clip]{figures/huggingface.png}
    \caption{Left: PromptGuard~\cite{promptguard}~\textsuperscript{1}, Right: ProtectAIv2~\cite{protectai}~\textsuperscript{2}, which is current SotA prompt guard model. We found that existing prompt guard models have an over-defense issue, i.e., misclassify benign inputs as malicious due to an overreliance on specific trigger words, such as ``ignore''.}
    \label{fig_toy_experiment}
\vspace{-0.3cm}
\end{figure*}

Despite these advantages, we find that existing prompt guard models face a critical limitation: the issue of over-defense. Over-defense arises when models misclassify inputs due to reliance on shortcuts, resulting in false positives where benign inputs are incorrectly flagged as threats. For instance, as shown in Fig.~\ref{fig_toy_experiment}, commonly used words such as ``ignore'' or ``cancel'' can be in part of harmless sentences but are misclassified as malicious by many existing (even commercial) prompt guard models. Such over-defense problem reduces LLM accessibility, as the prompt guard model may reject legitimate user requests and block access. It can also cause significant disruptions in real-world applications, particularly in interactive systems like virtual assistants~\cite{10.1145/3580305.3599572} and medical diagnostic tools~\cite{thirunavukarasu2023large}, where immediate and reliable access is crucial.

To address this issue, we introduce \textbf{\dataset}, an evaluation dataset specifically designed to assess the over-defense issue of existing models. The dataset contains 339 carefully crafted benign inputs, developed using statistical methods on existing benign and attack datasets. The test cases in \dataset contain trigger words commonly found in prompt injection attacks, while still preserving benign intent. We further divided the dataset into three levels of difficulty, based on the number of trigger words present, enabling more fine-grained evaluation. Through systematic evaluations based on \dataset, we demonstrate that current prompt guard models, including current \textit{state-of-the-art} (SotA) solutions like ProtectAIv2~\cite{protectai}, suffer from significant over-defense issues, with over-defense accuracy falling below 60\%, which is close to random guessing (50\%).

In addition to the dataset, we also propose (\textbf{\methodname}), which mitigates the above over-defense issue.  Since existing prompt guard models are closed-source and training data is not released, our journey starts with curating a comprehensive collection of training datasets with carefully designed data-centric augmentation techniques for addressing the long-tail problem. 
% for training and apply data-centric 358
% augmentation techniques to address the long-tail 359
% problem within the datase.
To further address the over-defense problem, instead of directly finetuning on a specific dataset (e.g,   \dataset), which introduces unfair evaluation results, 
here, we introduce \textit{Mitigating Over-defense for Free} (MOF), , without relying on any specific over-defense datasets.  As a result, \textbf{\modelname} achieves SotA performance across multiple benchmarks, including \dataset. Evaluation results show that \modelname~outperforms existing prompt guard models, achieving over 83\% average accuracy in detecting benign, malicious, and over-defense inputs, surpassing the runner-up prompt guard model by 30.8\%. Remarkably, \modelname~achieves similar performance to GPT-4o~\cite{gpt4o}, a commercial LLM, while being an lightweight model trained on DeBERTa~\cite{deberta}. Furthermore, our model reaches this performance using a fully open-source dataset, unlike some existing prompt guard models that rely on closed datasets~\cite{promptguard,protectai}, further promoting a transparency and open-source academic research environment.

\footnotetext[1]{\url{https://huggingface.co/meta-llama/Prompt-Guard-86M}}
\footnotetext[2]{\url{https://huggingface.co/protectai/deberta-v3-base-prompt-injection-v2}}

% , because they are also common \textit{trigger words} for prompt injection attacks.
% without requiring access to any additional over-defense datasets.

==> sections_ARR_submission/2-related-works.tex <==
\section{Related Works}\label{section_related}
\bsub{Prompt injection attacks.} Prompt injection attacks have become a critical threat to LLMs. Since LLMs process inputs in natural language, they often face challenges distinguishing between legitimate user commands and external manipulative inputs, leaving them vulnerable. The concept is first identified in research by~\citet{perez_ignore_2022}, revealing that LLMs could be misled by simple, crafted inputs, resulting in goal hijacking and prompt leakage. Several studies have been proposed~\cite{greshake_not_2023,wang_safeguarding_2023,pedro_prompt_2023,yan_backdooring_2023,yu_assessing_2023,salem_maatphor_2023,yip_novel_2024,zhan2024injecagentbenchmarkingindirectprompt,liu2024automatic,pasquini2024neuralexeclearningand,shi2024optimizationbasedpromptinjectionattack}, addressing various aspects of prompt injection attacks, such as handcrafted methods~\cite{toyer_tensor_2023}, automatic attack algorithms~\cite{liu2024automatic}, and benchmarks~\cite{liu_prompt_2023-1,debenedetti2024agentdojo}. Public discussions~\cite{rich2023prompt,pi_against_gpt3,delimiters_url} have also underscored the risks of prompt injection attacks on commercial LLMs. Prompt Injection datasets are also introduced, such as PINT-benchmark~\cite{pint}, Safeguard-Injection~\cite{safe_guard_prompt_injection}, Deepset-Injection~\cite{deepset_data}, TaskTracker~\cite{tasktracker}, and BIPIA~\cite{yi_benchmarking_2023}. 

\bsub{Prompt guard models.} Prompt guard models offer a promising approach to defend against prompt injection attacks by detecting malicious intent in inputs. These methods are computationally efficient and, unlike LLM guardrails~\cite{inan2023llamaguardllmbasedinputoutput}, do not require an additional round of victim LLM inference to generate a response. Several prompt guard models have been proposed recently. Fmops~\cite{fmops} is a guardrail trained by FmopsAI, utilizing DistilBERT~\cite{sanh2020distilbertdistilledversionbert} as the backbone. Deepset~\cite{deepset}, PromptGuard~\cite{promptguard}, and ProtectAIv2~\cite{protectai} all employ DeBERTaV3-base~\cite{deberta} as the backbone. Deepset~\cite{deepset} is trained on Deepset-Injection~\cite{deepset_data}, a small open-sourced dataset with 546 samples. PromptGuard is a model trained by Meta with a close-sourced dataset. ProtectAIv2 is also trained with a close-sourced dataset by Protect AI, achieving SotA performance on PINT-benchmark~\cite{pint}.

However, these prompt guard models suffer from over-defense issues, where they rely on shortcuts triggered by certain keywords to make predictions, leading them to incorrectly categorize a benign input that contains the keywords as malicious. Moreover, some of these models are trained using closed-source data~\cite{promptguard, protectai}. In this paper, we introduce an over-defense dataset to systematically evaluate the over-defense issue, and propose a novel training approach that achieves SotA performance across diverse benchmarks, including the over-defense dataset.

\begin{figure}[t!]
\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering    
    \includegraphics[width=0.45\textwidth,trim=0 0 0 0,clip]{figures/smooth_illustration.pdf}
    \caption{Visualization of attention weight. Given an instruction of ``[CLS] Can I ignore this warning appeared in my code? [SEP]'', ProtectAIv2~\cite{protectai} assigns extremely high attention weights to the word ``ignore,'' leading to misclassification as Injection. In contrast, our method distributes attention across the entire sentence, successfully predicting it as benign.}
    \label{fig_smooth}
\vspace{-0.3cm}
\end{figure}

==> sections_ARR_submission/3-dataset.tex <==
\section{Over-defense Dataset: \dataset}\label{sec_dataset}
% In this section, we will first identify the over-defense phenomenon that existing in many existing commercial guardrails \cite{}. To systematically evaluate this issue, we propose a benchmark\name \chaowei{xxx}, which covers xxx. 

% \begin{figure*}[t!]
% \setlength{\abovecaptionskip}{5pt}
% \setlength{\belowcaptionskip}{0pt}
% \centering
% \begin{subfigure}{0.48\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim=0 10 0 30,clip]{figures/PG.png}
%     \caption{PromptGuard~\footnote{\url{https://huggingface.co/meta-llama/Prompt-Guard-86M}}}
%     \label{fig:PG}
% \end{subfigure}
% \begin{subfigure}{0.48\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim=0 10 0 30,clip]{figures/protectAI.png}
%     \caption{ProtectAIv2~\footnote{\url{https://huggingface.co/protectai/deberta-v3-base-prompt-injection-v2}}}
%     \label{fig:protect}
% \end{subfigure}
% \caption{Existing prompt guard models have an over-defense issue, i.e., misclassify benign inputs as malicious due to an overreliance on specific trigger words, such as ``ignore''.}
% \vspace{-0.3cm}
% \label{fig_toy_experiment}
% \end{figure*}

\subsection{The Over-defense Issue}\label{sec_dataset_issue} 
While prompt guards offer several advantages, such as low overhead as previously mentioned, we have identified a critical limitation: they exhibit severe over-defense issues, even in some commercial tools~\cite{protectai}. Specifically, these models learn a shortcut from certain trigger words, like ``ignore'', directly to the final prediction. As shown in Fig.~\ref{fig_smooth} with red lines, ProtectAIv2~\cite{protectai}, one of the SOTA prompt guard models on PINT-benchmark, distributes excessive and unbalanced attention to the word ``ignore'', leading it to incorrectly categorize a benign input as malicious. To further illustrate this issue, we input a benign sentence containing the word ``ignore'' into two advanced prompt guard models: PromptGuard~\cite{promptguard} and ProtectAIv2~\cite{protectai}, and present the results in Fig.~\ref{fig_toy_experiment}. Both models incorrectly classify the benign instruction containing the word ``ignore'' as malicious.

% We believe the above toy experiment demonstrates the model's tendency to misclassify benign inputs as malicious due to an overreliance on specific trigger words. 
In this paper, \textbf{we define the over-defense issue} in prompt guard models as \textit{the tendency to predict malicious labels when benign sentences contain certain trigger words commonly used in prompt injection attacks}.
% these models tend to make final predictions based on only certain trigger words, such as trigger words like ``ignore'', rather than considering the entire sentence in context. To illustrate this issue, we input the word ``ignore'' into several prompt guard models and assess their predictions. Since this word alone does not imply any prompt injection intent, it should be classified as \lh{``benign''. However, as shown in Fig.~\ref{fig_tool_experiment}, } 
% \lh{Specifically, we select $2$ advanced prompt guard models of PromptGuard\footnote{https://huggingface.co/meta-llama/Prompt-Guard-86M} and ProtectAIv2\footnote{https://huggingface.co/protectai/deberta-v3-base-prompt-injection-v2}, which incorrectly predict the instruction containing the word of ``ignore'' as ``malicious''.} 

\begin{figure*}[t!]
\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering    
    \includegraphics[width=0.9\textwidth,trim=0 0 0 0,clip]{figures/pipeline.png}
    \caption{The pipeline for constructing \dataset~dataset.}
    \label{fig_dataset_pipeline}
\vspace{-0.3cm}
\end{figure*}

\subsection{Construction of \dataset}\label{sec_dataset_construction}
To enhance the community's ability to address the above issues, we introduce an over-defense evaluation dataset that supports systematically evaluating the over-defense issue inherent in prompt guard models. As shown in Fig.~\ref{fig_dataset_pipeline}, to build \dataset, there are three main steps: 1) Trigger word identification, which aims to find candidate trigger words likely to cause over-defense; 2) Trigger word refinement, which filters out misidentified words from the first step; and 3) Corpus generation, which uses LLMs to generate over-defense test cases based on the identified trigger words. 

% Next, we will describe each steps in details. 
% we first collect the trigger words that are widely used for prompt injection attacks and then build the evaluation corpus based on these trigger words.
 % , in this paper, we introduce an over-defense evaluation dataset \dataset. 
% This dataset is specifically designed to test models' accuracy to benign inputs that, while containing words commonly associated with prompt injections, are used in non-malicious contexts.

\bsub{Trigger Words Identification.} We begin by collecting two primary datasets: a dataset containing known prompt injection attack examples, denoted as $D_m$ (malicious dataset), and a benign dataset comprising typical user inputs devoid of malicious intent, denoted as $D_b$. We collect these data from several open-source datasets, such as Alpaca~\cite{alpaca} and Safeguard-Injection~\cite{safe_guard_prompt_injection} (detailed information is provided in the Appendix.~\ref{appendix_data}). The injection dataset includes various malicious inputs crafted to manipulate LLMs, whereas the benign dataset represents non-harmful user interactions. Then, as illustrated in Fig.~\ref{fig_dataset_pipeline}, we perform a word frequency analysis on both datasets. For each dataset, we compute the word frequencies to obtain frequency lists $F_b$ and $F_m$ for the benign and malicious datasets, respectively. We rank these words based on their frequencies from highest to lowest, resulting in two separate lists sorted by occurrence rates. Next, to identify injection-specific words, we compare the word frequency rank between the two datasets. By calculating the rank difference through, $\Delta r(w) = R_b(w) - R_m(w)$, we recognize words that are more frequent in the injection dataset but less common in the benign dataset. Words that exhibit a significantly higher frequency in the injection dataset are flagged as potential trigger words associated with prompt injections. Our detailed algorithm is shown in Alg.~\ref{alg_dataset}. We also visualize the top 20 words identified as trigger words by our method in Fig.~\ref{fig_frequency}.


\bsub{Trigger Words Refinement.} Recognizing that automated methods may include irrelevant or common words not indicative of prompt injection attempts, we proceed with a word rectification process. We first employ LLM to automatically filter the list of candidate words to remove any that may not be pertinent. Specifically, We assess the potential harmfulness of words by asking GPT-4o-mini (\citet{openai2024gpt4omini}, we use the 2024-07-18 version by default unless otherwise specified) questions like, ``Do you think the word of \textbf{\{word\}} is especially frequent in malicious or prompt attack scenarios?''~\textsuperscript{1} 
Next, we perform a manual verification step, where we review the remaining words after LLM filtering to ensure that any words unrelated to prompt injection attacks are removed. Through these two steps, we have compiled a word list with the highest potential for malicious use.
\begin{figure}[t]
\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering    
    \includegraphics[width=0.45\textwidth,trim=0 0 0 0,clip]{figures/freq.pdf}
    \caption{The top-20 rank differences between benign and malicious datasets.}
    \label{fig_frequency}
\vspace{-0.5cm}
\end{figure}
% This is followed by a manual verification step, where \lh{we scrutinize the remained words after filtering to ensure their appropriateness and relevance}\xg{should clarify that if you are looking at the word that is filtered out, or otherwise}, thus eliminating any false positives that may have been overlooked by the LLM. 
% \lh{Through these two steps of refinement, we have extracted a word list with the highest potential for malice.}

\bsub{Corpus Generation.} With a refined list of trigger words, we then generate sample sentences. We instruct the GPT-4o-mini to craft new sentences that must include a specified number of the selected trigger words~\textsuperscript{2}. Specifically, {we select the generated 113 trigger words and create three subsets with distinct difficulty levels, determined by the number of trigger words used in the generation of new sentences. Namely, three subsets separately containing 1, 2, and 3 trigger words are built with 113 benign sentences per subset. It is imperative that these sentences are contextually coherent, semantically meaningful, and do not contain any prompt injection instructions or malicious content. The goal is to represent benign usage of the trigger words in everyday language, ensuring that the sentences reflect natural and diverse linguistic patterns. To accomplish this, we design a carefully curated prompt (see Appendix.~\ref{sec_prompt}) to guide the LLM in generating safe and natural sentences. We then implement a polish process to further ensure the safety of the generated samples. In this process, the generated sentences are re-input into the LLM to identify any potential injection vulnerabilities, using the prompt detailed in Appendix.~\ref{sec_prompt}. Following this, we conduct a manual review to confirm the safety of all sentences. This multi-step refinement process guarantees that all generated sentences are harmless.
% \chaowei{How do we achieve it? We need to mention it? HOw can we ensure there is not harmful/injection instruction in our generated corpus?} 
The final output forms the proposed \dataset, which contains a total of 339 generated samples with 113 for one-word subset, 113 for two-word subset, and 113 for three-word subset.
% \chaowei{We need to add more details about it? What prompts are using for generating data?}
\renewcommand{\thefootnote}{}
\footnotetext{\textsuperscript{1, 2} Detailed prompts are in the Appendix.}
\renewcommand{\thefootnote}{\arabic{footnote}}

% which we carefully balance in terms of the number of samples containing different trigger words, as well as the distribution of sentence lengths and complexities. This balanced dataset serves as a robust tool for evaluating the over-defense behaviors of prompt guard models.
% By meticulously constructing this over-defense evaluation dataset, we provide a valuable resource for testing and improving prompt guard models. This dataset challenges models to accurately interpret inputs containing trigger words without overreacting to benign content. Consequently, it aids in reducing unnecessary blocking of legitimate user inputs and enhances the practical applicability of prompt guard systems.

\begin{algorithm}[h]
\begin{small}
\caption{\begin{small} Trigger Words Identification \end{small}}
\label{alg_dataset}
\begin{algorithmic}[1]
\Require Benign dataset $D_b$, Malicious dataset $D_m$, Integer $k$
% \Ensure Top $k$ words with the largest frequency differences
\State Compute word frequencies in $D_b$ to get frequency list $F_b$
\State Compute word frequencies in $D_m$ to get frequency list $F_m$
\State Sort $F_b$ in descending order to get rank list $R_b$
\State Sort $F_m$ in descending order to get rank list $R_m$
\ForAll{words $w$ in $R_b \cup R_m$}
    \State Compute rank difference $(\Delta r(w) = R_b(w) - R_m(w))$
    \State Add $(w, \Delta r(w))$ to list $L$
\EndFor
\State Sort list $L$ in descending order based on $\Delta f(w)$
% \State Initialize an empty list $L$ for storing frequency differences
% \ForAll{words $w$ in $F_b \cup F_m$}
%     \State Compute frequency difference $(\Delta f(w) = |F_b(w) - F_m(w)|)$
%     \State Add $(w, \Delta f(w))$ to list $L$
% \EndFor
% \State Sort list $L$ in descending order based on $\Delta f(w)$
\State \Return Top $k$ words from list $L$
\end{algorithmic}
\end{small}
\end{algorithm}

\subsection{Evaluations on \dataset}\label{sec_dataset_eval}
Here, we present our evaluations based on the proposed \dataset, assessing $4$ existing prompt guard models. To provide a comprehensive evaluation, in addition to the over-defense evaluation, we employ a three-dimensional metric. First, we measure \textit{malicious accuracy}, which reflects how effectively the models detect malicious inputs using attack data from the PINT-benchmark~\cite{pint} and BIPIA datasets~\cite{yi_benchmarking_2023}. Second, we evaluate \textit{benign accuracy}, i.e., how accurately the models classify benign data as non-malicious, using benign data from both the PINT-benchmark and WildGuard benchmark~\cite{wildguard}. Finally, we assess \textit{over-defense accuracy}, which captures the models' performance when encountering benign inputs that contain trigger words like ``ignore'', using our proposed \dataset~dataset.

\begin{figure}[t]
\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering    \includegraphics[width=0.48\textwidth,trim=50 10 40 30,clip]{figures/3D.pdf}
    \caption{Comparison on 3 dimensions of benign, malicious, and over-defense accuracy.}
    \label{fig_datset_eval}
\vspace{-0.3cm}
\end{figure}

% \lh{In Fig.~\ref{fig_datset_eval}, we explore the capabilities of several existing injection guard models in terms of benign, malicious, and over-defense scenarios.}
Based on above, we evaluate existing prompt guard models (i.e., Deepset~\cite{deepset}, Fmops~\cite{fmops}, PromptGuard~\cite{promptguard}, and ProtectAIv2~\cite{protectai}). 
% \chaowei{why do we miss llama, gpt4o here? why only such a imited model set? }


The results are shown in Fig.~\ref{fig_datset_eval}, where the x, y, and z axes represent malicious accuracy, benign accuracy, and over-defense accuracy, respectively. As illustrated, none of the existing prompt guard models (i.e., Deepset~\cite{deepset}, Fmops~\cite{fmops}, PromptGuard~\cite{promptguard}, and ProtectAIv2~\cite{protectai}) can achieve high accuracy across all three dimensions simultaneously. More importantly, none of the existing prompt guard models achieve an over-defense accuracy greater than $60\%$, where $50\%$ represents random guessing. These findings underscore that our \dataset~poses a significant challenge for current prompt guard models, effectively revealing the prevalent over-defense issue. This highlights the urgent need to develop a robust prompt guard model that excels in malicious accuracy, benign accuracy, and over-defense accuracy, with particular emphasis on addressing the over-defense issue.

==> sections_ARR_submission/4-method.tex <==
% \section{SotA Prompt Guard: \modelname}\label{sec_model}
\section{\modelname}\label{sec_model}

In this section, we aim to develop a robust prompt guard model that excels in malicious accuracy, benign accuracy, and over-defense accuracy. We also want to emphasize that many existing prompt guard models are closed-source and do not disclose their training data. Our objective is to train our model using only publicly available data, thereby promoting transparency and facilitating academic research. Here, we introduce \modelname, a prompt guard model that achieves state-of-the-art performance across various benchmarks. To build \modelname, we first curate a comprehensive collection of open-source datasets for training and apply data-centric augmentation techniques to address the long-tail problem within the dataset. More importantly, we propose a novel training strategy, \methodname, which effectively mitigates over-defense issues without relying on any specific over-defense datasets.

\subsection{Data Collection and Augmentation}\label{sec_model_training_data}

Similar to existing models, we first collect a wide range of prompt injection and benign corpus as the training data. 
% Specifically, we select $N$ open-source datasets, including the \textit{PromptBench} dataset \cite{promptbench}, the \textit{PI-Dataset} \cite{pidataset}, and the \textit{SafeText} corpus \cite{safetext}. These datasets encompass diverse input formats for LLMs, ensuring the effectiveness and generalization of our model.
Specifically, we select $22$ open-source datasets, including the benign datasets like Alpaca~\cite{alpaca}, the prompt injection datasets like Safeguard-Injection~\cite{safe_guard_prompt_injection}, and the datasets generated by existing injection attack, such as TaskTrack~\cite{tasktracker}). However, upon analyzing these datasets, we identify a long-tail issue in these datasets: certain input formats frequently exploited in prompt injection attacks—such as CSV files—are underrepresented. To address this, we implement a data-centric augmentation procedure, generating additional data for these long-tail formats. Using GPT-4o-mini, we create both benign and prompt injection samples in 17 formats, including Email, Document, Chat Conversation, JSON, Code, Markdown, HTML, URL, Base64, Table, XML, CSV, Config File, Log File, Image Link, Translation, and Website. After augmentation, our final training dataset for \modelname~comprises $55,893$ benign samples and $14,496$ prompt injection samples, where $434$ samples are generated by our data-centric augmentation procedure. Detailed statistics of the training data and prompt for data-centric augmentation are provided in the Appendix.~\ref{appendix_data} and Appendix.~\ref{sec_prompt}.

\subsection{\textit{Mitigating Over-defense for Free} (\methodname)}\label{sec_model_mitigating}
% As discussed in Sec.~\ref{sec_dataset_issue}, existing prompt guard models tend to make final predictions based solely on certain words rather than considering the entire input, leading to significant bias and over-defense issues.
To address the over-defense issue, we propose \textbf{M}itigating \textbf{O}ver-defense for \textbf{F}ree (\methodname), a novel method to identify and mitigate such biases, without relying on any specific over-defense datasets. 

Specifically, after training our model with the aforementioned data (Sec.~\ref{sec_model_training_data}) using standard supervised learning (training details are deferred to the Appendix), we perform a ``token-wised recheck'' to identify biases in the trained model. This procedure takes every token in the tokenizer vocabulary and inputs each token individually into the trained model. Ideally, these tokens should all be considered ``benign'' since they are individual tokens without any intent of prompt injection attack. By doing this, we can identify any biased words that are incorrectly predicted as ``attack'' by the model. We consider the bias toward these tokens as the root cause of the over-defense issue in the model.

After identifying the biased tokens, we prompt GPT-4o-mini to generate benign data using random combinations of these tokens (including one-token, two-token, and three-token settings, as mentioned in Sec.~\ref{sec_dataset_construction}). We generate 1,000 benign samples using this method. Subsequently, we incorporate these generated data into the training data introduced in Sec.~\ref{sec_model_training_data} to form the final training dataset. Using this dataset, we retrain our prompt guard model from scratch and get the final \modelname. 

% \bsub{Performance.} 
As illustrated in Fig.~\ref{fig_smooth}, the retrained model focuses and makes the final prediction on the overall meaning of the entire input, rather than certain trigger words. And results in Fig.~\ref{fig_datset_eval} show that our model achieves high accuracy across all three dimensions simultaneously. We also present ablation studies of the aforementioned training design in Tab.~\ref{tab_training_ablation}. More detailed evaluation results are provided in the following section.


==> sections_ARR_submission/5-experiments.tex <==
\section{Evaluations}\label{section_experiment}
% \begin{table*}[t!]
% \begin{center}{
% \setlength{\belowcaptionskip}{-0.1cm}
%   {
%   \setlength{\tabcolsep}{2pt}
%   \small
% \begin{tabular}{@{}llcccc@{}}
% \toprule
% \textbf{Category} & \textbf{Model}  & \textbf{Over-defense (\%)} & \textbf{Benign (\%)} & \textbf{Malicious (\%)} & \textbf{Average (\%)} \\ 
% \midrule
% \multirow{4}{*}{\textbf{Prompt Guard Model}} 
% & Fmops~\cite{fmops} & 5.60 & 34.63 & 93.50 & 44.58 \\
% & Deepset~\cite{deepset} & 5.31  & 34.06   & 91.50 & 43.62 \\
% & PromptGuard~\cite{promptguard} & 0.88 & 26.82 & 97.10 & 41.60 \\
% & ProtectAIv2~\cite{protectai} & 56.64 & 86.20 & 48.60 & 63.81 \\
% \midrule
% \multirow{3}{*}{\textbf{Large Language Model}} 
% & GPT-4o~\cite{gpt4o} & 86.73 & 90.78 & 79.10 & 85.53 \\
% & Llama-2-chat~\cite{touvron2023llama} & 76.40 & 61.03 & 31.09 & 56.17 \\
% & LlamaGuard3~\cite{dubey2024llama3herdmodels} & 99.71 & \textbf95.18 & 28.28 & 74.39 \\
% \midrule
% \multirow{1}{*}{\textbf{Prompt Guard Model}} & \modelname~(Ours) & 87.32 & 85.74 & 77.39 & 83.48 \\
% \bottomrule
% \end{tabular}}
% }
% \vspace{-0.2cm}
% \caption{Accuracy comparison between our model, \modelname, and other baseline models. \modelname~surpasses the runner-up (ProtectAIv2) by 30.8\% in terms of average accuracy. Additionally, \modelname~achieves performance comparable to GPT-4o, a commercial LLM, despite being an open-source model trained on DeBERTa.}
% \vspace{-0.3cm}
% \label{tab_main_results}%
% \end{center}
% \end{table*}%

% \begin{table*}[h]
% \centering
% \begin{center}{
% \setlength{\belowcaptionskip}{-0.1cm}
%   {
%   \setlength{\tabcolsep}{2pt}
%   \small
% \begin{tabular}{l|cccc}
% \hline
% \multirow{2}{*}{\textbf{Method}}         & \multicolumn{4}{c}{\textbf{Over-defense}} \\  
% \cmidrule(lr){2-5}
%                         & \textbf{one-word} & \textbf{two-word} & \textbf{three-word} & \textbf{average}\\
%                        \hline
% Deepset        & 5.31    & 7.08    & 3.54 & 5.31\\ 
% Fmops          & 5.31    & 5.31    & 6.19  & 5.60 \\ 
% PromptGuard    & 2.65    & 0.00       & 0.00 & 0.88  \\ 
% ProtectAIv2    & 76.11   & 47.79   & 46.02  & 56.64 \\ 
% GPT-4o         & 95.58   & 85.84   & 78.76  &  86.73  \\ 
% Llama-2-chat   & 82.3    & 79.65   & 67.26  & 76.4 \\ 
% LlamaGuard3    & 100.00     & 100.00     & 99.12  & 99.71 \\ 
% \textbf{InjecGuard (Ours)} & 91.15 & 89.38   & 81.42 & 87.32\\
% \hline
% \end{tabular}
% }}
% \vspace{-0.2cm}
% \caption{Results on the three levels of difficulties in \dataset.}
% \vspace{-0.3cm}
% \label{tab_over_defense}
% \end{center}
% \end{table*}

\begin{table*}[t!]
\begin{center}{
\setlength{\belowcaptionskip}{-0.1cm}
  {
  \setlength{\tabcolsep}{0.5pt}
  \scriptsize
\begin{tabular}{@{}llcccc|ccc@{}}
\toprule
 &   & \multicolumn{4}{c|}{\textbf{Performance}} & \multicolumn{3}{c}{\textbf{Overhead}}\\
 \cmidrule{3-6}\cmidrule{7-9}
 \textbf{Category} & \textbf{Model} & \textbf{Over-defense (\%)} & \textbf{Benign (\%)} & \textbf{Malicious (\%)} & \textbf{Average (\%)} & \textbf{GFLOPs} & \textbf{Inference (ms)} & \textbf{Efficiency} \\ 
\midrule
\multirow{4}{*}{\textbf{Prompt Guard Model}} 
& Fmops~\cite{fmops} & 5.60 & 34.63 & 93.50 & 44.58 & 24.19 & 4.43 & 10.06\\
& Deepset~\cite{deepset} & 5.31  & 34.06   & 91.50 & 43.62 & 60.45 & 15.22 & 2.87\\
& PromptGuard~\cite{promptguard} & 0.88 & 26.82 & 97.10 & 41.60 & 60.45 & 15.28 & 2.72\\
& ProtectAIv2~\cite{protectai} & 56.64 & 86.20 & 48.60 & 63.81 & 60.45 & 15.77 & 4.05\\
\midrule
\multirow{3}{*}{\textbf{Large Language Model}} 
& GPT-4o~\cite{gpt4o} & 86.73 & 90.78 & 79.10 & 85.53  & - & 7907.18 & 0.01\\
& Llama-2-chat~\cite{touvron2023llama} & 76.40 & 61.03 & 31.09 & 56.17 & 1387.49 & 3111.36  & 0.02 \\
& LlamaGuard3~\cite{dubey2024llama3herdmodels} & 99.71 & \textbf95.18 & 28.28 & 74.39 & 1418.38 & 787.48 & 0.09\\
\midrule
\multirow{1}{*}{\textbf{Prompt Guard Model}} & \modelname~(Ours) & 87.32 & 85.74 & 77.39 & 83.48 & 60.45 & 15.34  & 5.44 \\
\bottomrule
\end{tabular}}
}
\vspace{-0.2cm}
\caption{Performance and overhead comparison between our model, \modelname, and other baseline models. \modelname~surpasses the runner-up (ProtectAIv2) by 30.8\% in terms of average accuracy. Additionally, \modelname~achieves performance comparable to GPT-4o, a commercial LLM, despite being an lightweight model trained on open-source data. We calculate the Efficiency = Average Accuracy/Inference Time.}
\vspace{-0.5cm}
\label{tab_main_results}%
\end{center}
\end{table*}%

\subsection{Experimental Setups}\label{experiment_settings}
\bsub{Evaluation Datasets.} As mentioned in Sec.~\ref{sec_dataset_eval}, we conduct our evaluations based on three aspects: benign accuracy, malicious accuracy, and over-defense accuracy. To fully verify the practicality of our proposed \modelname, we ensure that all evaluation datasets are not included in the training data. Specifically, For evaluating the benign accuracy, we utilize benign data from both the Pint-Benchmark and WildGuard benchmark~\cite{wildguard}. For evaluating the malicious accuracy, We use attack data from both the PINT-Benchmark~\cite{pint} and BIPIA datasets~\cite{yi_benchmarking_2023}. For evaluating the over-defense accuracy, we use the proposed \dataset~dataset.

\vspace{0.1cm}
\bsub{Metrics.} Since prompt guard models function as text classification systems that predict whether an input text is benign or malicious, we evaluate their performance using \textit{Accuracy}, calculated as the proportion of correct predictions over the total number of test cases in the evaluation dataset:

\begin{small}
\begin{equation}
    \text{Accuracy} = \frac{\text{Number of Correct Predictions}}{\text{Total Number of Test Cases}}
\end{equation}
\end{small}
Additionally, we report the computational overhead in terms of \textit{Giga Floating Point Operations} (GFLOPs), which quantifies the total number of floating-point operations required during inference. GFLOPs provide an estimate of the computational resources needed by the model. We also measure the \textit{inference time} to assess the computational overhead introduced by the models.

\bsub{Training Details of \modelname.} We employ DeBERTaV3-base~\citep{deberta} as the backbone of \modelname and train it with a batch size of 32 for 3 epochs, using Adam~\cite{adam} optimizer and linear scheduler. The initial learning rate is set to 2e-5, with a 100-step warm-up phase. Besides, the maximum token length is set to 512.

\bsub{Baselines.} We employ four existing prompt guard models as baselines: Fmops~\cite{fmops}, Deepset~\cite{deepset}, PromptGuard~\cite{promptguard}, and ProtectAIv2~\cite{protectai}, which are introduced in Sec.~\ref{section_related}. We also consider LLM-based methods, including LlamaGuard3~\cite{dubey2024llama3herdmodels}, Llama-2-chat-7b~\cite{touvron2023llama}, and GPT-4o~\cite{gpt4o}, which are evaluated by prompting them to determine a given input constitutes a prompt injection attack.

% \begin{figure}[h]
% \setlength{\abovecaptionskip}{5pt}   
% \setlength{\belowcaptionskip}{0pt}
%     \centering    \includegraphics[width=0.45\textwidth,trim=0 0 0 0,clip]{figures/smooth_illustration.pdf}
%     \caption{Comparison of attention weight. Given an instruction of ``[CLS] Can I ignore this warning appeared in my code? [SEP]'', ProtectAIv2 assigns extremely high attention weights to the word "ignore," leading to a misclassification as Injection. In contrast, our method distributes attention across the entire sentence, successfully predicting it as benign.}
%     \label{fig_smooth}
% \vspace{-0.3cm}
% \end{figure}

% \begin{table*}[t!]
% \begin{center}{
% \setlength{\belowcaptionskip}{-0.1cm}
%   {
%   \setlength{\tabcolsep}{3pt}
%   \small
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% Model  & \textbf{GFLOPS} & \textbf{Inference time (ms)} & \textbf{Performance (\%)} & \textbf{Efficiency (Performance/Inference time)} \\ 
% \midrule
% Fmops & 24.19  & 4.43  & 44.58 & 10.06 \\
% Deepset & 60.45  & 15.22  & 43.62 & 2.87\\
% PromptGuard & 60.45  & 15.28  & 41.60 & 2.72 \\
% ProtectAIv2 & 60.45  & 15.77  & 63.81 & 4.05 \\
% GPT-4o & - & 7907.18 & 85.53 & 0.01 \\
% Llama-2-chat & 1387.49  & 3111.36  & 56.17 & 0.02 \\
% LlamaGuard3 & 1418.38  & 787.74  & 74.39 & 0.09 \\
% \midrule
% \modelname~(Ours) & 60.45  & 15.34  & 83.48 & \textbf{5.44} \\
% \bottomrule
% \end{tabular}
% }}
% \vspace{-0.2cm}
% \caption{Comparison of Computational Overhead.}
% \vspace{-0.3cm}
% \label{tab_complexity}%
% \end{center}
% \end{table*}

\subsection{Main Results}
The comparison results of our method and other baselines are shown in Tab.~\ref{tab_main_results}. Our \modelname~demonstrates superior performance compared to existing prompt guard models and even rivals commercial LLMs like GPT-4o. Specifically, \modelname~achieves an average accuracy of 83.48\%, surpassing the runner-up prompt guard baseline (ProtectAIv2) by 30.83\%. Our model excels across all evaluation categories, attaining an over-defense accuracy of 87.32\%, benign accuracy of 85.74\%, and malicious accuracy of 77.39\%. This balanced performance indicates that \modelname~is highly effective at correctly identifying benign and malicious inputs while minimizing false positives and negatives. The fact that \modelname~achieves results comparable to GPT-4o, despite being based on the open-source data and lightweight backbone, highlights the efficiency and effectiveness of our training approach. Notably, according to Tab.~\ref{tab_main_results}, the Efficiency (Performance/Inference time) of our model is 503 times higher than that of GPT-4o.

The results also prove that existing prompt guard models suffer from overwhelming issues with over-defense, as reflected by their low over-defense accuracy scores. Models like Fmops, Deepset, and PromptGuard exhibit over-defense accuracies as low as 5.60\%, 5.31\%, and 0.88\%, respectively, indicating a tendency to incorrectly classify benign inputs that have trigger words as malicious. And ProtectAIv2 has an over-defense accuracy of 56.64\%, which is close to random guessing (50.00\%). This issue underscores the challenges posed by our proposed over-defense dataset. In addition, the superior over-defense accuracy of \modelname~demonstrates its robustness in this field. The over-defense accuracy of our \modelname~surpasses the runner-up prompt guard model (ProtectAIv2) by 54.17\%, showing that our model effectively handles the challenging cases presented by the dataset, and confirming the efficacy of our novel training approach \methodname~in mitigating over-defense issues prevalent in existing models. Note that \methodname~does not require any over-defense dataset for training; instead, it automatically generates adaptive training data, verifying it as both practical and highly effective.

\begin{table*}[t!]
\begin{center}{
\setlength{\belowcaptionskip}{-0.1cm}
  {
  \setlength{\tabcolsep}{6pt}
  \small
\begin{tabular}{@{}lcccc@{}}
\toprule
Training Design  & \textbf{Over-defense (\%)} & \textbf{Benign (\%)} & \textbf{Malicious (\%)}  & \textbf{Average (\%)} \\ 
\midrule
\rowcolor{myblue} Training on the Basic Dataset (Sec.~\ref{sec_model_training_data}) & 75.22  & 78.53   & 70.17 &  74.64 \\
\rowcolor{myred} \quad + Data-centric Augmentation (Sec.~\ref{sec_model_training_data})          & 64.31  & 81.36   & 75.95  &  73.87 \\
\midrule
\rowcolor{myblue} Training on the Basic Dataset (Sec.~\ref{sec_model_training_data}) & 75.22  & 78.53   & 70.17 &  74.64 \\
\rowcolor{mygreen} \quad + MOF with Retraining from Scratch (Sec.~\ref{sec_model_mitigating})     & \textbf{89.38}  & 84.73   & 71.57  &  81.89 \\
\midrule
\rowcolor{myblue} Training on the Basic Dataset (Sec.~\ref{sec_model_training_data}) & 75.22  & 78.53   & 70.17 &  74.64 \\
\rowcolor{myred} \quad + Data-centric Augmentation (Sec.~\ref{sec_model_training_data})          & 64.31  & 81.36   & 75.95  &  73.87 \\
\rowcolor{mygreen} \quad + MOF with Finetuning (Sec.~\ref{sec_model_mitigating})         & 68.14  & 82.11   & 74.81 &  75.02 \\
\midrule
\rowcolor{myblue} Training on the Basic Dataset (Sec.~\ref{sec_model_training_data}) & 75.22  & 78.53   & 70.17 &  74.64 \\
\rowcolor{myred} \quad + Data-centric Augmentation (Sec.~\ref{sec_model_training_data})          & 64.31  & 81.36   & 75.95  &  73.87 \\
\rowcolor{mygreen} \quad + MOF with Retraining from Scratch (Sec.~\ref{sec_model_mitigating})        & 87.32   & \textbf{85.74}   & \textbf{77.39} & \textbf{83.48} \\
\bottomrule
\end{tabular}}
}
\vspace{-0.2cm}
\caption{Ablation study of each training design introduced in Sec.~\ref{sec_model}.}
\vspace{-0.5cm}
\label{tab_training_ablation}%
\end{center}
\end{table*}

\subsection{Ablation Studies}
The ablation study presented in Tab.~\ref{tab_training_ablation} offers key insights into the effects of our training components on \modelname performance. Starting with the Basic Dataset, the model establishes a baseline average accuracy of 74.64\%, with over-defense, benign, and malicious accuracies of 75.22\%, 78.53\%, and 70.17\%, respectively. Introducing Data-centric Augmentation alone leads to a noticeable improvement in benign accuracy (from 78.53\% to 81.36\%) and malicious accuracy (from 70.17\% to 75.95\%), enhancing the model’s ability to correctly classify both benign and malicious inputs. However, this augmentation comes at a cost, as evidenced by a significant reduction in over-defense accuracy from 75.22\% to 64.31\%. This decline indicates that while data-centric augmentation enriches the training data and improves classification capabilities, it inadvertently exacerbates the over-defense issue, making the model more prone to incorrectly classifying benign inputs as malicious—a challenge commonly observed in existing models.

The introduction of the \methodname, particularly when combined with Retraining from Scratch, addresses the adverse effects of data-centric augmentation on over-defense accuracy. Applying MOF with Retraining from Scratch to the Basic Dataset lifts the average accuracy to 81.89\%, with over-defense, benign, and malicious accuracies at 89.38\%, 84.73\%, and 71.57\%, respectively. This substantial improvement highlights MOF's effectiveness in mitigating over-defense issues caused by data-centric augmentation. When both Data-centric Augmentation and MOF with Retraining from Scratch are used, the model achieves the highest average accuracy of 83.48\%, with over-defense, benign, and malicious accuracies of 87.32\%, 85.74\%, and 77.39\%. This combination leverages the strengths of both data augmentation and mitigation strategies, resulting in a robust model that not only benefits from enhanced classification performance but also maintains high over-defense accuracy. The ablation study demonstrates that data-centric augmentation alone can improve certain aspects of model performance, and the integration of MOF techniques is essential to counterbalance the increased over-defense, thereby ensuring that \modelname~achieves optimal and balanced performance across all metrics.

\subsection{Computational Overhead}
% Our model \modelname~demonstrates exceptional computational efficiency while delivering superior performance compared to existing baseline models. As illustrated in Tab.~\ref{tab_main_results}, \modelname~achieves an impressive average accuracy of 83.48\%. This enhancement in performance does not come at the cost of increased computational resources. \modelname~maintains a GFLOPS count of 60.45, identical to several other prompt guard models, and an inference time of merely 15.34 milliseconds. Moreover, our model boasts the highest efficiency score of 5.44, calculated as the ratio of performance to inference time, underscoring its ability to deliver robust results swiftly and resource-effectively. This balance of high accuracy and low computational overhead makes \modelname~a highly attractive solution for deployment in environments where both performance and efficiency are paramount.

% In contrast, while LLMs such as GPT-4o exhibit commendable performance levels, their substantial computational demands render them less practical for certain applications where operational efficiency is needed. GPT-4o, for instance, achieves an accuracy of 85.53\%, which is comparable to \modelname; however, it does so with an exorbitant inference time of 7907.18 milliseconds, leading to an efficiency score of merely 0.01. Similarly, other LLM-based models like Llama-2-chat and LlamaGuard3 require thousands of GFLOPS and prolonged inference times, resulting in efficiency scores that are orders of magnitude lower than \modelname. This significant disparity highlights the impracticality of deploying such LLMs in scenarios where computational resources and response times are critical constraints. In contrast, \modelname offers a highly effective and efficient alternative, making it better for real-world applications that demand both high accuracy and efficiency.
Our model, \modelname, excels in both computational efficiency and performance compared to existing baseline models. As shown in Table~\ref{tab_main_results}, \modelname~ achieves an average accuracy of 83.48\% while maintaining a GFLOPS count of 60.45 and an inference time of only 15.34 milliseconds. With an efficiency score of 5.44 (performance divided by inference time), \modelname~delivers robust results swiftly and resource-effectively, making it ideal for environments prioritizing both accuracy and efficiency. In contrast, LLMs like GPT-4o achieve slightly higher accuracy (85.53\%) but at a significant computational cost, with an inference time of 7907.18 milliseconds and an efficiency score of 0.01. Similarly, models such as Llama-2-chat and LlamaGuard3 require thousands of GFLOPS and longer inference times, resulting in much lower efficiency. This disparity highlights the impracticality of deploying these LLMs in scenarios where computational resources and quick response times are essential. Therefore, \modelname~presents a highly effective and efficient alternative for real-world applications demanding both high accuracy and operational efficiency.



==> sections_ARR_submission/6-conclusions.tex <==
\section{Conclusions}
In this study, we delved into the over-defense phenomenon observed in existing injection-based prompt guard models. To address this issue, we proposed a novel over-defense data sampling framework and introduced the NotInject benchmark to systematically evaluate the extent of over-defense in target prompt guard models. Furthermore, we presented InjecAgent, an advanced prompt guard model trained using a novel robust training strategy, MOF, designed to effectively mitigate model bias toward specific words. Our experimental results on various benchmark demonstrate that InjecAgent significantly outperforms existing prompt guard models across multiple dimensions, with substantial improvements in performance and robustness.

\newpage
\section*{Limitations}
While our work shows significant improvement in mitigating over-defense in prompt guard models, the \dataset~dataset, while carefully designed, may not fully capture the diversity of real-world benign inputs, particularly in domain-specific applications. This could result in the underestimation of models' over-defense tendency in complex, sensitive fields such as healthcare or finance. However, as our comprehensive evaluations have shown, the current design of \dataset~is sufficient to reveal the over-defense issue in existing prompt guard models, highlighting the urgent need for improved approaches in this community. To further enhance the diversity of \dataset, our future work will incorporate domain-specific data through collaboration with industry partners.

\section*{Ethics Statement}
We are committed to advancing the security and integrity of LLMs responsibly. In this research, we introduce \dataset, a dataset designed to assess and mitigate the over-defense issue in prompt guard models. Additionally, we introduce \modelname, a powerful prompt guard model developed using our novel approach, \methodname, aimed at enhancing LLM security. All data used are synthetically generated or sourced from publicly available datasets, ensuring that no personal or sensitive information is involved. This approach safeguards privacy and complies with ethical standards regarding data use.

While our work focuses on enhancing defensive mechanisms against prompt injection attacks, we acknowledge the potential for dual use in security research. We encourage the ethical and responsible use of \dataset~to improve LLM security and not for malicious purposes. By addressing over-defense, we aim to reduce false positives and enhance accessibility for all users when prompt guard models are deployed. Our commitment to transparency is reflected in making both the dataset and model fully open-source, fostering collaboration, and allowing others to verify, replicate, and build upon our work for the betterment of the field.
